Reproducibility of machine learning analyses of 21 cm reionization maps

Machine learning (ML) methods have become popular for parameter inference in cosmology, although their reliance on specific training data can cause difficulties when applied across different data sets. By reproducing and testing networks previously used in the field, and applied to 21cmFast and Simfast21 simulations, we show that convolutional neural networks (CNNs) often learn to identify features of individual simulation boxes rather than the underlying physics, limiting their applicability to real observations. We examine the prediction of the neutral fraction and astrophysical parameters from 21 cm maps and find that networks typically fail to generalise to unseen simulations. We explore a number of case studies to highlight factors that improve or degrade network performance. These results emphasise the responsibility on users to ensure ML models are applied correctly in 21 cm cosmology.

==> still_todo.tex <==
% Holding location for comments and corrections that are needed in the text
% but that don't fit easily into the main documents

Use the \TBC{this} tag to add in text that is based on missing figures or things that will need to be discussed carefully with KS for accuracy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

* Polish abstract for paper

* Key result figures need to be rescaled to show the correct parameter values and not the normalised values that are used in the training process.

* Missing two results figures for section 4.3.
These are (1) the plot of predicted vs true ionization fraction for the network trained and tested on slices from the same set of boxes and (2) the equivalent plot where the network is tested on slices from newly simulated boxes that appear nowhere in the training set. Then we need more text to explain what these results show - provisionally that the network is able to work on the newly simulated boxes and so is able to predict the ionization fraction from unseen boxes. This is an indication that the network is able to generalise to unknown data.

* Figure 9:
    * Ideally we'd include the corresponding point from Figure 8 (for 1 slice per box)
    * It would be good to colour the points corresponding to Figure 7 & 8 and label them in the caption. Then add some discussion of those specific cases in the main text.

* Bibliography needs some checking to see that we've captured the most recent papers looking at CNNs applied to 21cm. I think there are more than we've included at present, so be good to take a pass through and see what might be missing.

* Some references for the Simfast21 and excursion set formalism need to be filled in where there are placeholder \cite{} commands

* remove figure files that are no longer needed for the paper

* All plots need borders - MNRAS instructions "Where a figure has several parts, labels (a), (b) etc. should be added as appropriate. Figures (plots) containing quantitative information should have borders on all sides and fiducial marks on every border. Axes should be labelled and include the units. "
